Beyond 2:4: exploring V:N:M sparsity for efficient transformer inference on GPUs

To date, 2:4 sparsity has stood as the only sparse pattern that can be accelerated using sparse tensor cores on GPUs. In practice, 2:4 sparsity often possesses low actual speedups ($\leq 1.3$) and requires fixed sparse ratios, meaning that other ratios, such as 4:8, 8:16, or those exceeding 50% sparsity, do not incur any speedups on GPUs. Recent studies suggest that V:N:M sparsity is promising in addressing these limitations of 2:4 sparsity. However, regarding accuracy, the effects of V:N:M sparsity on broader Transformer models, such as vision Transformers and large language models (LLMs), are largely unexamined. Moreover, Some specific issues related to V:N:M sparsity, such as how to select appropriate V and M values, remain unresolved. In this study, we thoroughly investigate the application of V:N:M sparsity in vision models and LLMs across multiple tasks, from pertaining to downstream tasks. We propose three key approaches to enhance the applicability and accuracy of V:N:M-sparse Transformers, including heuristic V and M selection, V:N:M-specific channel permutation, and three-staged LoRA training techniques. Experimental results show that, with our methods, the DeiT-small achieves lossless accuracy at 64:2:5 sparsity, while the DeiT-base maintains accuracy even at 64:2:8 sparsity. In addition, the fine-tuned LLama2-7B at 64:2:5 sparsity performs comparably or better than training-free 2:4 sparse alternatives on downstream tasks. More importantly, V:N:M-sparse Transformers offer a wider range of speedup-accuracy trade-offs compared to 2:4 sparsity. Overall, our exploration largely facilitates the V:N:M sparsity to act as a truly effective acceleration solution for Transformers in cost-sensitive inference scenarios.

==> common_tmp.tex <==
\usepackage{color}
\usepackage{bm}
\usepackage{hyperref}
\usepackage{amsmath,amsfonts,amsthm}
\usepackage{blindtext}
\usepackage{listings}
\usepackage{algorithm, algorithmic}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{caption}
\usepackage{enumitem} % 加了这个包就work了，是否该加
% \usepackage{subcaption}


\newcommand{\quant}[1]{Q\left(#1\right)}

% ======= Latin =======
\newcommand{\naive}{na\"{i}ve}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}


\newlist{myitems}{enumerate}{3}
\setlist[myitems, 1]
{label=\arabic{myitemsi}.,leftmargin=15pt,labelwidth=10pt,labelsep=5pt,
topsep=0pt,parsep=0pt,partopsep=0pt,noitemsep
}

\newcommand{\hqmm}{\texttt{HQ-MM}}
\newcommand{\lssmm}{\texttt{LSS-MM}}


% ======= Comments =======


% Conditionals (for draft mode)
\usepackage{ifthen}

%%%%%%%%%%%%%
%%% Change between \commentstrue and \commentsfalse to remove large margins and ocmments
\newif\ifdebug
% \debugtrue
\debugfalse

\newcommand{\baohan}[1]{{\color{blue}{\bf\sf [Baohan: #1]}}}
\newcommand{\yuantao}[1]{{\color{purple}{\bf\sf [Yuantao: #1]}}}
\newcommand{\zhaokang}[1]{{\color{green}{\bf\sf [ZhaoKang: #1]}}}
\newcommand{\jianfei}[1]{{\color{red}{\bf\sf [Jianfei: #1]}}}
% \newcommand{\joey}[1]{{\color{red}{\bf\sf [Joey: #1]}}}
% \else
% \newcommand{\jianfei}[1]{{\color{red}{}
% }}
% \newcommand{\joey}[1]{{\color{red}{}}}
% \fi
% \newcommand{\michael}[1]{{\leavevmode\color{red}{Michael:\ #1}}}
\newcommand{\bingrui}[1]{{\color{blue}{\bf\sf [Bingrui: #1]}}}
\newcommand{\lily}[1]{{\color{blue}{\bf\sf [Lily: #1]}}}


% ======= Theorem =======

\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\round}[1]{\left\lfloor #1 \right\rceil}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\tofloat}[1]{\mbox{float}\left(#1\right)}
\newcommand{\toint}[2]{\mbox{int}_{#1}\left(#2\right)}

% ======= Misc math =======
\newcommand{\qf}[1]{Q_f\left(#1\right)}
\newcommand{\qa}[1]{Q_f\left(#1\right)}
\newcommand{\qt}[1]{Q_{\theta}\left(#1\right)}
%\newcommand{\qb}[1]{Q_b\left(#1\right)}
\newcommand{\qb}[1]{Q_b(#1)}
\newcommand{\Hl}[1]{{\Hv^{(#1)}}}
\newcommand{\Dl}[1]{{D^{(#1)}}}
\newcommand{\tHl}[1]{{\tilde \Hv}^{(#1)}}
\newcommand{\hl}[1]{{\hv_i^{(#1)}}}
\newcommand{\thl}[1]{{{\tilde \hv}_i^{(#1)}}}
\newcommand{\hkl}[1]{{\hv_k^{(#1)}}}
\newcommand{\El}[1]{{\epsilonv^{(#1)}}}
\newcommand{\ekl}[1]{{\epsilonv_k^{(#1)}}}
\newcommand{\W}[1]{{\Wv^{(#1)}}}
\newcommand{\Thetal}[1]{{\Thetav^{(#1)}}}
\newcommand{\T}[1]{{\Tv^{(#1)}}}
\newcommand{\tW}[1]{\mbox{${\tilde \Wv}^{(#1)}$}}
\newcommand{\tT}[1]{\mbox{${\tilde \Thetav}^{(#1)}$}}
\newcommand{\tb}[1]{\mbox{${\tilde \bv}^{(#1)}$}}
\newcommand{\F}[2]{{\Fv^{(#1)}}\left(#2\right)}
\newcommand{\G}[2]{{\Gv^{(#1)}}\left(#2\right)}
\newcommand{\f}[2]{{\fv^{(#1)}}\left(#2\right)}
\newcommand{\hn}{\hat\nabla}
\newcommand{\tn}{\tilde\nabla}
\newcommand{\Jl}{\Jv^{(l)}}
\newcommand{\Kl}{\Kv^{(l)}}
\newcommand{\jikl}{\Jv_{ik}^{(l)}}
\newcommand{\Kkl}{\Kv_{k}^{(l)}}
\newcommand{\jiil}{\Jv_{ii}^{(l)}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\SR}{\mathtt{SR}}
\newcommand{\R}{\mathrm{R}}
\newcommand{\ssl}{S^{(l)}}
\newcommand{\zl}{Z^{(l)}}

\newcommand{\vect}[1]{\boldsymbol{\mathbf{#1}}}

\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

\newcommand{\quantize}[1]{Q\left(#1\right)}

% \newcommand{\Mean}{\mbox{Mean}}
\newcommand{\ve}[1]{\mathrm{vec}(#1)}
\newcommand{\vecinv}{\mathrm{vec}^{-1}}
\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\Econd}[2]{\mathbb{E}\left[#1\;\middle|\;#2\right]}
\newcommand{\Var}[1]{\mathrm{Var}\left[#1\right]}
\newcommand{\Cov}[2]{\mathrm{Cov}\left[#1,#2\right]}
\newcommand{\Mean}[1]{\mathrm{Mean}\left[#1\right]}
\newcommand{\VarF}[1]{\mathrm{Var}\left[#1\right]}
\newcommand{\Varcond}[2]{\mathrm{Var}\left[#1\;\middle|\;#2\right]}
\newcommand{\VarFcond}[2]{\mathrm{Var}\left[#1\;\middle|\;#2\right]}
\newcommand{\Std}[1]{\mathrm{Std}\left[#1\right]}
\newcommand{\N}{\mathcal{N}}
\newcommand{\Bern}{\mbox{Bern}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\Mult}{\mbox{Mult}}
\newcommand{\Unif}{\mbox{Unif}}
\newcommand{\Cat}{\mbox{Cat}}
\newcommand{\dx}{\mbox{d}x}
\newcommand{\dy}{\mbox{d}y}

% ======= Greek letters =======
\newcommand{\alphav}{\vect\alpha}
\newcommand{\betav}{\vect\beta}
\newcommand{\gammav}{\vect\gamma}
\newcommand{\deltav}{\vect\delta}
\newcommand{\epsilonv}{\vect\epsilon}
\newcommand{\zetav}{\vect\zeta}
\newcommand{\etav}{\vect\eta}
\newcommand{\thetav}{\vect\theta}
\newcommand{\iotav}{\vect\iota}
\newcommand{\kappav}{\vect\kappa}
\newcommand{\lambdav}{\vect\lambda}
\newcommand{\muv}{\vect\mu}
\newcommand{\nuv}{\vect\nu}
\newcommand{\xiv}{\vect\xi}
\newcommand{\omicronv}{\vect\omicron}
\newcommand{\piv}{\vect\pi}
\newcommand{\rhov}{\vect\rho}
\newcommand{\sigmav}{\vect\sigma}
\newcommand{\tauv}{\vect\tau}
\newcommand{\upsilonv}{\vect\upsilon}
\newcommand{\phiv}{\vect\phi}
\newcommand{\chiv}{\vect\chi}
\newcommand{\psiv}{\vect\psi}
\newcommand{\omegav}{\vect\omega}

\newcommand{\Alphav}{\vect\Alpha}
\newcommand{\Betav}{\vect\Beta}
\newcommand{\Gammav}{\vect\Gamma}
\newcommand{\Deltav}{\vect\Delta}
\newcommand{\Epsilonv}{\vect\Epsilon}
\newcommand{\Zetav}{\vect\Zeta}
\newcommand{\Etav}{\vect\Eta}
\newcommand{\Thetav}{\vect\Theta}
\newcommand{\Iotav}{\vect\Iota}
\newcommand{\Kappav}{\vect\Kappa}
\newcommand{\Lambdav}{\vect\Lambda}
\newcommand{\Muv}{\vect\Mu}
\newcommand{\Nuv}{\vect\Nu}
\newcommand{\Xiv}{\vect\Xi}
\newcommand{\Omicronv}{\vect\Omicron}
\newcommand{\Piv}{\vect\Pi}
\newcommand{\Rhov}{\vect\Rho}
\newcommand{\Sigmav}{\vect\Sigma}
\newcommand{\Tauv}{\vect\Tau}
\newcommand{\Upsilonv}{\vect\Upsilon}
\newcommand{\Phiv}{\vect\Phi}
\newcommand{\Chiv}{\vect\Chi}
\newcommand{\Psiv}{\vect\Psi}
\newcommand{\Omegav}{\vect\Omega}

% ======= English letters =======
\newcommand{\av}{\vect a}
\newcommand{\bv}{\vect b}
\newcommand{\cv}{\vect c}
\newcommand{\dv}{\vect d}
\newcommand{\ev}{\vect e}
\newcommand{\fv}{\vect f}
\newcommand{\gv}{\vect g}
\newcommand{\hv}{\vect h}
\newcommand{\iv}{\vect i}
\newcommand{\jv}{\vect j}
\newcommand{\kv}{\vect k}
\newcommand{\lv}{\vect l}
\newcommand{\mv}{\vect m}
\newcommand{\nv}{\vect n}
\newcommand{\ov}{\vect o}
\newcommand{\pv}{\vect p}
\newcommand{\qv}{\vect q}
\newcommand{\rv}{\vect r}
\newcommand{\sv}{\vect s}
\newcommand{\tv}{\vect t}
\newcommand{\uv}{\vect u}
\newcommand{\vv}{\vect v}
\newcommand{\wv}{\vect w}
\newcommand{\xv}{\vect x}
\newcommand{\yv}{\vect y}
\newcommand{\zv}{\vect z}

\newcommand{\Av}{\vect A}
\newcommand{\Bv}{\vect B}
\newcommand{\Cv}{\vect C}
\newcommand{\Dv}{\vect D}
\newcommand{\Ev}{\vect E}
\newcommand{\Fv}{\vect F}
\newcommand{\Gv}{\vect G}
\newcommand{\Hv}{\vect H}
\newcommand{\Iv}{\vect I}
\newcommand{\Jv}{\vect J}
\newcommand{\Kv}{\vect K}
\newcommand{\Lv}{\vect L}
\newcommand{\Mv}{\vect M}
\newcommand{\Nv}{\vect N}
\newcommand{\Ov}{\vect O}
\newcommand{\Pv}{\vect P}
\newcommand{\Qv}{\vect Q}
\newcommand{\Rv}{\vect R}
\newcommand{\Sv}{\vect S}
\newcommand{\Tv}{\vect T}
\newcommand{\Uv}{\vect U}
\newcommand{\Vv}{\vect V}
\newcommand{\Wv}{\vect W}
\newcommand{\Xv}{\vect X}
\newcommand{\Yv}{\vect Y}
\newcommand{\Zv}{\vect Z}

\newcommand{\Ac}{\mathcal A}
\newcommand{\Bc}{\mathcal B}
\newcommand{\Cc}{\mathcal C}
\newcommand{\Dc}{\mathcal D}
\newcommand{\Ec}{\mathcal E}
\newcommand{\Fc}{\mathcal F}
\newcommand{\Gc}{\mathcal G}
\newcommand{\Hc}{\mathcal H}
\newcommand{\Ic}{\mathcal I}
\newcommand{\Jc}{\mathcal J}
\newcommand{\Kc}{\mathcal K}
\newcommand{\Lc}{\mathcal L}
\newcommand{\Mc}{\mathcal M}
\newcommand{\Nc}{\mathcal N}
\newcommand{\Oc}{\mathcal O}
\newcommand{\Pc}{\mathcal P}
\newcommand{\Qc}{\mathcal Q}
\newcommand{\Rc}{\mathcal R}
\newcommand{\Sc}{\mathcal S}
\newcommand{\Tc}{\mathcal T}
\newcommand{\Uc}{\mathcal U}
\newcommand{\Vc}{\mathcal V}
\newcommand{\Wc}{\mathcal W}
\newcommand{\Xc}{\mathcal X}
\newcommand{\Yc}{\mathcal Y}
\newcommand{\Zc}{\mathcal Z}

\newcommand{\Ab}{\mathbb A}
\newcommand{\Bb}{\mathbb B}
\newcommand{\Cb}{\mathbb C}
\newcommand{\Db}{\mathbb D}
\newcommand{\Eb}{\mathbb E}
\newcommand{\Fb}{\mathbb F}
\newcommand{\Gb}{\mathbb G}
\newcommand{\Hb}{\mathbb H}
\newcommand{\Ib}{\mathbb I}
\newcommand{\Jb}{\mathbb J}
\newcommand{\Kb}{\mathbb K}
\newcommand{\Lb}{\mathbb L}
\newcommand{\Mb}{\mathbb M}
\newcommand{\Nb}{\mathbb N}
\newcommand{\Ob}{\mathbb O}
\newcommand{\Pb}{\mathbb P}
\newcommand{\Qb}{\mathbb Q}
\newcommand{\Rb}{\mathbb R}
\newcommand{\Sb}{\mathbb S}
\newcommand{\Tb}{\mathbb T}
\newcommand{\Ub}{\mathbb U}
\newcommand{\Vb}{\mathbb V}
\newcommand{\Wb}{\mathbb W}
\newcommand{\Xb}{\mathbb X}
\newcommand{\Yb}{\mathbb Y}
\newcommand{\Zb}{\mathbb Z}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\inorm}[1]{\norm{#1}_\infty}
\newcommand{\iprod}[1]{\langle#1\rangle}


\newcommand{\cvloss}{f_{CV, v}}
\newcommand{\loss}{f_v}
\newcommand{\ZL}{Z^{(l)}}
\newcommand{\ZLp}{Z^{(l+1)}}
\newcommand{\HL}{H^{(l)}}
\newcommand{\HLp}{H^{(l+1)}}
\newcommand{\scv}{_{CV}}
\newcommand{\ZLcv}{\ZL\scv}
\newcommand{\ZLpcv}{\ZLp\scv}
\newcommand{\HLcv}{\HL\scv}
\newcommand{\HLpcv}{\HLp\scv}
\newcommand{\WL}{W^{(l)}}
\newcommand{\WLT}{W^{(l)\top}}
\newcommand{\PhL}{\hat P^{(l)}}
\newcommand{\diag}{\mbox{diag}}

\newcommand{\vp}{{v^\prime}}
\newcommand{\bl}{{(l)}}
\newcommand{\bll}{{(l+1)}}
\newcommand{\bL}{{(L)}}
\newcommand{\NS}{\mbox{NS}}
\newcommand{\CV}{\mbox{CV}}
\newcommand{\CVD}{\mbox{CVD}}
\newcommand{\Ideal}{\mbox{Ideal}}
\newcommand{\nbr}{\nv(u)}
\newcommand{\snbr}{\hat \nv^\bl(u)}
\newcommand{\var}[2]{\Var_{#1}\left[#2\right]}

\newcommand{\rh}{\mathring{h}}
\newcommand{\tr}[1]{\mbox{tr}\left(#1\right)}



\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
	\newenvironment{rep#1}[1]{%
		\def\rep@title{#2 \ref{##1}}%
		\begin{rep@theorem}}%
		{\end{rep@theorem}}}
\makeatother




\newcommand{\hst}{\hat s_t}
\newcommand{\hstt}{\hat s_{t+1}}
\newcommand{\Dfhst}{\Delta f_i(\hst)}
\newcommand{\bfhst}{\bar f(\hst)}
\newcommand{\bfhstt}{\bar f(\hstt)}
\newcommand{\bhstt}{\bar s_{t+1}}
\newcommand{\grad}[1]{\nabla_{#1} f(#1)}
\newcommand{\hess}[1]{\nabla^2_{#1} f(#1)}
\newcommand{\lmax}{\lambda_{\mbox{max}}}
\newcommand{\lmin}{\lambda_{\mbox{min}}}
\newcommand{\hsz}{\hat s_0}
\newcommand{\Uniform}{\mbox{Uniform}}

\newcommand{\Zl}{\mathbf{1} \zv^{(l)}}
\newcommand{\Sl}{\Sv^{(l)}}
\newcommand{\Slinv}{(\Sv^{(l)})^{-1}}

==> text/backup.tex <==
Notably, V:N:M-specific CP is exclusively applied to feed-forward networks (FFNs) in a Transformer since only the CP of FFNs can be fully absorbed without increasing time costs during inference. To be specific, given an input $\Xv$, CP for a FFN are represented as:
\begin{equation}
FFN(\Xv,\Pv) = \Wv_2\Pv^\top (ReLU(\Pv\Wv_1 \Xv + \bv_1)) + \bv_2,
\label{eq:cpffn}
\end{equation}
where $\Wv_1 \in\Rb^{d_o\times d_i}$ ,$\Wv_2 \in\Rb^{d_i\times d_o}$, and $\Pv \in\Rb^{d_o\times d_o}$. $\Pv$ is a permutation matrix. Due to $\Pv^\top\Pv=\Iv$, it is evident that FFN(\Xv,\Pv)=FFN(\Xv).  
Besides, $\Pv\Wv_1$ and $\Wv_2\Pv$ can be calculated offline, thus not introducing extra overheads in inference.        

CP for 2:4 and V:N:M sparsity is different. In 2:4 sparsity, only input CP of a weight matrix influences the retained weight norm after pruning. In contrast, V:N:M sparsity allows both input and output CP to affect the retained weight norm. Thus for Eq. \ref{eq:cpffn}, Concentrating solely on optimally permuting the output channels of $\Wv_1$ during solving $\Pv$ may lead to unsatisfactory outcomes when $\Pv$ is applied to the input channels of $\Wv_2$. Besides, due to the large dimensions of input and output channels, searching viable $\Pv$ is time-consuming.

To address the issue, our V:N:M-specific CP approach solves permutation matrics block-wise and selectively. 1). Extract blocks from $\Wv_1$ and $\Wv_2$. 
The block size is the multiple of V*M so   2) Calculate two permutation matrices of the extracted block. 3) Selection. 4) Iteration.
%要指出llama还有个gate_proj

%sparse weight-mask co-optimization的
%In this work, the logic of calculating $\Mv$ is fairly straightforward. First, each weight in a weight matrix is depicted by an importance score. RIA is used to calculate the importance score since it is simple and can effectively retain the outlier weights \citep{zhang2024plug}. Secondly, in each V$\times$M block of a weight matrix, the importance score norm of each column is calculated, and the columns with the last M$-4$ small norms are pruned, e.g., red framed section in Figure \ref{fig:compare}. Lastly, in each row, the remaining weights with the last 2 small importance scores are pruned.          

% Second, the sparse masks are updated less frequently, specifically every 5 epochs instead of the 1 iteration per update reported in the original approach. Empirical evidence suggests that this reduced update frequency enhances training stability, ultimately resulting in improved final accuracy for V:N:M sparse Transformers.

